Playable Environments: Video Manipulation in Space and Time

We present Playable Environments - a new representation for interactive video generation and manipulation in space and time. With a single image at inference time, our novel framework allows the user to move objects in 3D while generating a video by providing a sequence of desired actions. The actions are learnt in an unsupervised manner. The camera can be controlled to get the desired viewpoint. Our method builds an environment state for each frame, which can be manipulated by our proposed action module and decoded back to the image space with volumetric rendering. To support diverse appearances of objects, we extend neural radiance fields with style-based modulation. Our method trains on a collection of various monocular videos requiring only the estimated camera parameters and 2D object locations. To set a challenging benchmark, we introduce two large scale video datasets with significant camera movements. As evidenced by our experiments, playable environments enable several creative applications not attainable by prior video synthesis works, including playable 3D video generation, stylization and manipulation. Further details, code and examples are available at https://willi-menapace.github.io/playable-environments-website

==> introduction_bak_12_nov.tex <==
\section{Introduction}

\setlength{\belowcaptionskip}{0pt}
\begin{figure}
    \centering
    \includegraphics[trim=0 0 0 14, clip,width=\columnwidth]{resources/teaser.pdf}

    %\caption{%\textbf{A playable environment for a tennis match}. 
    %Given a single initial frame, our method, named XXX, allows the user to interactively generate \emph{playable environments}, i.e. different videos by specifying discrete actions to control players, manipulating camera trajectory and indicating the style for each object in the scene.}
    \caption{%\textbf{A playable environment for a tennis match}. 
    Given a single initial frame, our method, named XXX, creates \emph{playable environments} that allow the user to interactively generate different videos by specifying discrete actions to control players, manipulating camera trajectory and indicating the style for each object in the scene.}
    \label{fig:teaser}
\end{figure}

% Version 2: 
What would you change in the last tennis match you saw? The actions of the player? The style of the field, or, perhaps, the camera trajectory to observe a highlight more dramatically \eli{i would remove fig 1 reference here}
(Fig.~\ref{fig:teaser})? To do so \eli{automatically???,}, % for tennis matches,
the geometry and the style of the field and the players need to be reconstructed. Players' actions need to be understood and the outcomes of future actions anticipated. To enable these features one needs to re-create the \emph{environment} in 3D and expose it in a way to provide simple and intuitive interaction as if the environment was \emph{playable}.
% \eli{do we need the next question?} How would the movement to the right look? % probably not
% To enable these features, one needs to understand the scene and expose it in a way 
% that is interactive and easy to manipulate. Moreover, the environment should provide 
% to provide simple and intuitive interaction
% , similar to that of a video-game, 
% as if the environment was \emph{playable}.
%Moreover, we would like to interact with this environment with the simplicity with which we can interact with a video-game, as if it was \emph{playable}.

Should such \emph{Playable Environment} of a video be constructed, multiple creative applications are unlocked, such as 3D- and action-aware video editing, camera trajectory manipulation, changing the action sequence, the agents and their styles, or continuing the video in time, beyond the observed footage.
% 
%At inference time our method can manipulate a previously unseen image or a video. 

\eli{stronger sentence here: tackle for the first time...}
In this work, we propose a method to construct Playable Environments (PE) from a single image. \eli{the single image here is only because we talk about inference but it is misleading}
Fig. \ref{fig:teaser} shows a playable environment for tennis matches built from a single image. In it, the user can specify actions and move the players, control the viewpoint and change the style of the players and the field. Thus the environment can be played, akin to a video game, but with real objects while being inferred from a single, previously unseen image.

The key contribution \eli{the following are not contributions} of our method are the six defining characteristics listed in Tab.~\ref{table:requirements}.
Our framework allows the user to interactively generate videos by providing discrete actions $\langle$\textbf{1}$\rangle$ and controlling the camera pose $\langle$\textbf{2}$\rangle$. Our method is trained on a dataset of diverse monocular videos, with multiple objects $\langle$\textbf{3}$\rangle$ with varying poses $\langle$\textbf{4}$\rangle$ and appearances $\langle$\textbf{5}$\rangle$. \eli{to give relevance of how we train here seems weird}
In addition, our framework is robust to imprecise inputs $\langle$\textbf{6}$\rangle$---we do not require ground-truth camera intrinsics and extrinsincs, but assume they can be estimated for each frame. Neither do we assume ground-truth object locations, but rely on an off-the-shelf object detector \cite{ren2015faster} to locate the agents in 2D, such as both tennis players.
% We do not require ground-truth camera intrinsics and extrinsincs, but assume they can be estimated for each frame $\langle$\textbf{6}$\rangle$. Finally, we assume there exists an off-the-shelf object detector \cite{ren2015faster} to locate the agents in 2D, such as both tennis players $\langle$\textbf{6}$\rangle$. 

% \eli{it is missing a clear distinction among new problem and new framework} \sergey{I think the problem is not new, DriveGAN, GameGAN and so on are trying to do so, our approach is new though}

Playable Environments \sergey{encapsulate and extend} several prior image or video manipulation problems. %Manipulating videos is  a long-standing problem in computer vision and graphics communities. 
%Multiple works attempt it from different perspectives. 
Novel view synthesis and volumetric rendering methods \eli{missign citations} support re-rendering of static scenes. However, with rare exceptions [], such methods do not support moving or articulated objects \sout{$\langle$\textbf{3}-\textbf{5}$\rangle$} and do not allow user interaction \sout{$\langle$\textbf{1}$\rangle$}, making them undesirable for modeling compelling environments. Video synthesis methods manipulate videos by predicting future frames \cite{lee2018savp,kumar2020videoflow,tulyakov2018moco,tian2021good}, animating~\cite{siarohin2019monkeynet,Siarohin2019firstorder,siarohin2021motion} or playing videos \cite{menapace2021pvg}, but environments modeled with such methods typically lack camera control and multi-object support \sout{$\langle$\textbf{2,3}$\rangle$}. Consequently, these methods limit interactivity as they do not take into account the 3D nature of the environment. 

\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize

\begin{tabular}{lp{0.08\textwidth}p{0.35\textwidth}}
\toprule
\bf  &\bf Name& \bf Description\\
\midrule
$\langle$\textbf{1}$\rangle$ &\textit{Playability} & The user can control generation with discrete actions.\\
$\langle$\textbf{2}$\rangle$ & \textit{Camera control} & The camera pose is explicitly controlled at test time.\\
$\langle$\textbf{3}$\rangle$ & \textit{Multi-object}& Each object is explicitly modeled. \\
$\langle$\textbf{4}$\rangle$& \textit{Deformable objects} & The model handles deformable object such as human body\\
$\langle$\textbf{5}$\rangle$ & \textit{Appearance changes} & The model handles objects whose appearance is not constant is the training set \\
$\langle$\textbf{6}$\rangle$ & \textit{Robustness} & The model is robust to calibration and localization errors.\\

\bottomrule
\end{tabular}
\end{center}
\caption{ Characteristics of our Playable Environments \eli{to me these are the caracteristics of the method and not of the problem}. Each row is referred in the text with $\langle \cdot \rangle$ symbols.}

\label{table:requirements}
\end{table}
%\vlad{Move this paragraph before the previous one? Otherwise, we talk about our method, then about existing techniques, then about our method again. }  
%\sergey{Actually this is intentional, I thought to introduce the method broadly, explain what we do. At that point the reader might say that other works do that too, hence this paragraphs shows the differences, then we give slightly more details about our method.}



%\vlad{In the following, NeRF should be introduced with more details by saying smth.~like ``Recently, coordinate-based neural volumentric representations gained attention. They do XXX and enable YYY... This paper adapts/proposes NeRF-based components for ZZZ.'' } 

Our method consists of two components. The first one is the synthesis module. It extracts the state of the environment---location, style and non-rigid pose of each object---and renders the state back to the image space. Recently introduced Neural Radiance Fields (NeRFs)~\cite{mildenhall2020nerf} represent an attractive vehicle for their ability to render novel views. 
% They employ a coordinate-based neural volumentric representation that enables novel view synthesis with an unprecedented quality. \sergey{I think this sentences is not needed}
In this work, we introduce a style-based modification of NeRF to support objects of different appearances. 
% Instead of rendering radiance directly and similarly to[], we compose image features decoded by a CNN. 
Furthermore, we propose a compositional non-rigid volumetric rendering approach handling the rigid parts of the scene and non-rigid objects. 
The second component---the action module---enables playability. It takes two consecutive states of the environment and predicts an action with respect to the camera orientation. We train our framework using reconstruction losses in the image space and the state space. Finally, to improve temporal dynamics, we introduce a temporal discriminator that operates on sequences of environment states. 
% 
%To evaluate playability, Menapace et al.~\cite{menapace2021pvg} use a 2D dataset of tennis matches. Since our playable environments are 3D, we introduce 2 newly collected datasets with camera movements. A large scale tennis dataset consisting of 43 tennis matches and the Minecraft Camera dataset. Furthermore, our method unlocks creative applications, such as real-video re-rendering, re-playing, object appearance manipulation and predicting future frames---all in a playable fashion. %The code, data and pre-trained models will be released to the community.
% 

To evaluate our method, we collected two large-scale datasets for the training of playable environment models of complex scenes and perform extensive quantitative and qualitative evaluation with several baselines derived from existing NeRF and video generation methods. These experiments show that our method is able to generate high quality videos and outperforms all baselines in terms of playability, camera control and video quality.


In summary, the primary contributions of this work are as follows: 
\begin{itemize}\itemsep0em  
    \item \eli{to me a new problem here} A new framework for the creation of compelling playable environments from a single image featuring six defining characteristics (see Tab.~\ref{table:requirements}). 
    \item  \eli{to me a new method here} A new compositional NeRF that handles deformable objects with different visual style and a new training strategy \eli{the new traning strategy is too specific considering that people may not know PVG since we do not discussed} for the action module that shows higher video quality and improved playability. 
    \item Two new large-scale datasets that allow training of {Playable  Environments}. A \emph{Minecraft} dataset with synthetic ground truth and a dataset of broadcasted \emph{Tennis} matches. \eli{stronger here, for future research in this novel problem bla bla}
\end{itemize}

\eli{As for PVG I would have name for the problem and a name for the method. this helps to disambiguate, also I would have acronym for PE}

%\vlad{Also currently missing: a short summary of the experimental results. Mention that our method enables functionality which none of the existing techniques can demonstrate. Mention briefly how we compare our method against existing methods, e.g., our method convinces in a user study, etc.} 

%\vlad{Any promise to release the source code and the new dataset?} 

% Can such reasoning be performed by a model trained on a set of diverse videos? In this paper we present a method to do this. At inference time given an image or a video it builds a playable environment that features aforementioned capabilities. Fig X shows an environment constructed by our method. In it, with the help of a set of actions the user a set of actions to move tennis players, use arrows to move the camera to change a view point and change the style of the player and the field. 




% Capabilities to change, manipulate, re-render and stylize recorded footage  extensive usage in movie and game industry. They require understanding of 

% Contrasting:
% - from volumetric rendering and novel view synthesis
% - from animation
% - from PVG

% From idea to tools, or from existing works by contrast?

% We present a framework 

% Key points:
% - Novel view sytnethsis with dynamic objects
% - Ability to play and control objects
% - Ability to change the style
% - "Do as I say"?

% How about this?

% There should a be good intro paragraph
% Videos represent verbatim recollection of events. They show environments in which they are recorded, with their geometry and style. They include objects that freely move and perform actions. 

% Videos represent events as they happened. It's not about videos, it's about enviroment

% Consider a tennis match. Broadcast involve sophisticated computer graphics to change the camera view, replay key events to create a more dramatic experience. A further interesting this is what could have been happened.



==> introduction_old_willi_edits.tex <==
\section{Introduction}

\setlength{\belowcaptionskip}{0pt}
\begin{figure}
    \centering
    \includegraphics[trim=0 0 0 14, clip,width=\columnwidth]{resources/teaser.pdf}

    %\caption{%\textbf{A playable environment for a tennis match}. 
    %Given a single initial frame, our method, named XXX, allows the user to interactively generate \emph{playable environments}, i.e. different videos by specifying discrete actions to control players, manipulating camera trajectory and indicating the style for each object in the scene.}
    \caption{%\textbf{A playable environment for a tennis match}. 
    We introduce the task of creating playable environments from a single initial frame.
    Our method, named XXX, creates playable environments that allow the user to generate different videos interactively by specifying discrete actions to control players, manipulating camera trajectory and indicating the style for each object in the scene.}
    \label{fig:teaser}
\end{figure}


% Version 3: 
What would you change in the last tennis match you saw? The actions of the player? The style of the field, or, perhaps, the camera trajectory to observe a highlight more dramatically \eli{in detail?}
(Fig.~\ref{fig:teaser})? To do so, % for tennis matches,
the geometry and the style of the field and the players need to be reconstructed. Players interact with the environment, and, hence, their past actions need to be understood and the outcomes of future actions anticipated. \eli{do we need the next question?} How would the movement to the right look?

% DEFINITION OF PLAYABLE ENVIRONMENT PROBLEM
In this work we introduce the problem of creating such \emph{playable environments} which consists in the creation from a single image of environments with the following capabilities: (i) \emph{Playability} the user can control generation with discrete actions; (ii) \emph{Camera control} the user can control the camera pose; (iii) \emph{Varying appearance} the environment can be built from datasets with objects of varied appearances.
An example of a playable environment of tennis matches is shown in Fig.~\ref{fig:teaser}. In it, the user can specify actions and move the player, control the viewpoint and change the style of the player and the field. Thus the environment can be played, akin to a video game, but with real objects while being inferred from a single, previously unseen image.
%APPLICATIONS OF PLAYABLE ENVIRONMENTS
With such playable environment of a video, multiple creative applications are unlocked, such as 3D- and action-aware video editing, camera trajectory manipulation, changing the action sequence, the agents and their styles. Furthermore, playable environments enable continuing the video in time, beyond the observed footage.

% RELATED PROBLEMS
Playable environments are closely related to several image or video manipulation problems. %Manipulating videos is  a long-standing problem in computer vision and graphics communities. 
%Multiple works attempt it from different perspectives. 
Novel view synthesis and volumetric rendering methods \eli{missing citations} support re-rendering of static scenes. However, with rare exceptions [], such methods do not support dynamic scenes with moving or articulated objects and do not allow user interaction. On the other hand, video synthesis methods manipulate videos by predicting future frames \cite{lee2018savp,kumar2020videoflow,tulyakov2018moco,tian2021good}, animating~\cite{siarohin2019monkeynet,Siarohin2019firstorder,siarohin2021motion} or playing videos \cite{menapace2021pvg} but limit interactivity as they do not take into account the 3D nature of the environment. Consequently, these methods fail to meet the characteristics of playable environments.

% CHARACTERISTICS OF OUR FRAMEWORK
In this work, we propose a method to construct playable environments from a single image.
%At inference time our method can manipulate a previously unseen image or a video. 
% \sergey{Our proposed playable environments feature the capabilities listed in Tab.~\ref{table:requirements}
%To support such interactive capabilities, our playable environments feature characteristics listed in Tab.~\ref{table:requirements}.}
% More specifically, playable environements meet the requirements listed in Tab.~\ref{table:requirements}.
At inference time, our framework allows the user to interactively generate videos by providing discrete actions and controlling the camera pose. Our method is trained on a dataset of diverse monocular videos, with multiple objects with varying poses and appearances and allows explicit control over the style of hte objects in the environment. 
\sergey{Our framework is robust to imprecise inputs ---we do not require ground-truth camera intrinsics and extrinsincs, but assume they can be estimated for each frame. Neither do we assume ground-truth object locations, but rely on an off-the-shelf object detector \cite{ren2015faster} to locate the agents in 2D, such as both tennis players.}
\vlad{imprecise inputs $\rightarrow$ noisy inputs; results not entirely meeting the assumptions of the method} 
% We do not require ground-truth camera intrinsics and extrinsincs, but assume they can be estimated for each frame $\langle$\textbf{6}$\rangle$. Finally, we assume there exists an off-the-shelf object detector \cite{ren2015faster} to locate the agents in 2D, such as both tennis players $\langle$\textbf{6}$\rangle$. 


%\vlad{Move this paragraph before the previous one? Otherwise, we talk about our method, then about existing techniques, then about our method again. }  
%\sergey{Actually this is intentional, I thought to introduce the method broadly, explain what we do. At that point the reader might say that other works do that too, hence this paragraphs shows the differences, then we give slightly more details about our method.}



%\vlad{In the following, NeRF should be introduced with more details by saying smth.~like ``Recently, coordinate-based neural volumentric representations gained attention. They do XXX and enable YYY... This paper adapts/proposes NeRF-based components for ZZZ.'' } 

% OUR FRAMEWORK
Our method consists of two components. The first one is the synthesis module. It extracts the state of the environment---location, style and non-rigid pose of each object---and renders the state back to the image space under a given camera pose. Recently introduced Neural Radiance Fields (NeRFs)~\cite{mildenhall2020nerf} represent an attractive vehicle for their ability and render novel views. They employ a coordinate-based neural volumentric representation that enables novel view synthesis with an unprecedented quality. In this work, we introduce style-based modulations of NeRF to support objects of different appearances. 
% Instead of rendering radiance directly and similarly to[], we compose image features decoded by a CNN.
Furthermore, we introduce a compositional non-rigid volumetric rendering approach that enables handling the rigid (e.g. field) and non-rigid (e.g. players) objects. 
The second component---the action module---enables playability. It takes two consecutive states of the environment and predicts an action with respect to the camera orientation. We train our framework using reconstruction losses in image space and the state space. Finally, to improve temporal dynamics, we introduce a temporal discriminator that operates on sequences of environment states. 
% 
%To evaluate playability, Menapace et al.~\cite{menapace2021pvg} use a 2D dataset of tennis matches. Since our playable environments are 3D, we introduce 2 newly collected datasets with camera movements. A large scale tennis dataset consisting of 43 tennis matches and the Minecraft Camera dataset. Furthermore, our method unlocks creative applications, such as real-video re-rendering, re-playing, object appearance manipulation and predicting future frames---all in a playable fashion. %The code, data and pre-trained models will be released to the community.
% 

We release two large-scale datasets for the training of playable environment models and perform extensive quantitative and qualitative evaluation with several baselines derived from existing NeRF and video generation methods. These experiments show that our methods is able to generate high quality videos and outperforms all baselines in terms of playability, camera control and video quality.

In summary, the primary contributions of this work are as follows: 
\begin{itemize}\itemsep0em
    \item The new problem of playable environment creation
    \item A new framework for the creation of playable environments from a single image. Our framework features a synthesis module with a compositional NeRF that handles input noise, deformable objects and diverse object appearances that shows higher video quality. Furthermore, we propose a new training strategy for the action module that improves playability. 
    \item Two new large-scale datasets that allow training of {Playable  Environments} methods. A \emph{Minecraft} dataset with synthetic ground truth and a dataset of broadcasted \emph{Tennis} matches. 
\end{itemize} 

\vlad{perhaps: few words about the experiments} 

%\vlad{Also currently missing: a short summary of the experimental results. Mention that our method enables functionality which none of the existing techniques can demonstrate. Mention briefly how we compare our method against existing methods, e.g., our method convinces in a user study, etc.} 


% Can such reasoning be performed by a model trained on a set of diverse videos? In this paper we present a method to do this. At inference time given an image or a video it builds a playable environment that features aforementioned capabilities. Fig X shows an environment constructed by our method. In it, with the help of a set of actions the user a set of actions to move tennis players, use arrows to move the camera to change a view point and change the style of the player and the field. 




% Capabilities to change, manipulate, re-render and stylize recorded footage  extensive usage in movie and game industry. They require understanding of 

% Contrasting:
% - from volumetric rendering and novel view synthesis
% - from animation
% - from PVG

% From idea to tools, or from existing works by contrast?

% We present a framework 

% Key points:
% - Novel view sytnethsis with dynamic objects
% - Ability to play and control objects
% - Ability to change the style
% - "Do as I say"?

% How about this?

% There should a be good intro paragraph
% Videos represent verbatim recollection of events. They show environments in which they are recorded, with their geometry and style. They include objects that freely move and perform actions. 

% Videos represent events as they happened. It's not about videos, it's about enviroment

% Consider a tennis match. Broadcast involve sophisticated computer graphics to change the camera view, replay key events to create a more dramatic experience. A further interesting this is what could have been happened.



==> introduction_original_bak.tex <==
\section{Introduction}

\setlength{\belowcaptionskip}{0pt}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{resources/teaser.pdf}

    %\caption{%\textbf{A playable environment for a tennis match}. 
    %Given a single initial frame, our method, named XXX, allows the user to interactively generate \emph{playable environments}, i.e. different videos by specifying discrete actions to control players, manipulating camera trajectory and indicating the style for each object in the scene.}
    \caption{%\textbf{A playable environment for a tennis match}. 
    Given a single initial frame, our method, named XXX, \sout{allows the user to interactively} creates \emph{playable environments} \willi{that allow the user to generate different videos interactively} by specifying discrete actions to control players, manipulating camera trajectory and indicating the style for each object in the scene.}
    \label{fig:teaser}
\end{figure}


\vlad{The paper starts like a novella. Unconventional but i am not against it.} \eli{i like it}
% Version 2: 
What would you change in the last tennis match you saw? The actions of the player? The style of the field, or, perhaps, the camera trajectory to observe a highlight more dramatically \eli{in detail?}
(Fig.~\ref{fig:teaser})? To do so, % for tennis matches,
the geometry and the style of the field and the players need to be reconstructed. Players interact with the \emph{environment}, and, hence, their past actions need to be understood and the outcomes of future actions anticipated. \eli{do we need the next question?} How would the movement to the right look? Should such \emph{playable environment} of a video be constructed, multiple creative applications are unlocked, such as 3D- and action-aware video editing, camera trajectory manipulation, changing the action sequence, the agents and their styles. Such a playable environment further enables continuing the video in time, beyond the observed footage.

In this work, we propose a method to construct Playable Environments from a single image.
%At inference time our method can manipulate a previously unseen image or a video. 
Fig. \ref{fig:teaser} shows an environment constructed by our method. In it, the user can specify actions and move the player, control the viewpoint and change the style of the player and the field. Thus the environment can be played, akin to a video game, but with real objects while being inferred from a single, previously unseen image.
\eli{it is missing a clear distinction among new problem and new framework}

\sergey{
% Our proposed playable environments feature the capabilities listed in Tab.~\ref{table:requirements}
To support such interactive capabilities, our playable environments feature characteristics listed in Tab.~\ref{table:requirements}.}
% More specifically, playable environements meet the requirements listed in Tab.~\ref{table:requirements}.
Our framework allows the user to interactively generate videos by providing discrete actions $\langle$\textbf{1}$\rangle$ and controlling the camera pose $\langle$\textbf{2}$\rangle$. Our method is trained on a dataset of diverse monocular videos, with multiple objects $\langle$\textbf{3}$\rangle$ with varying poses $\langle$\textbf{4}$\rangle$ and appearances $\langle$\textbf{5}$\rangle$. 
\sergey{Our framework is robust to imprecise inputs $\langle$\textbf{6}$\rangle$---we do not require ground-truth camera intrinsics and extrinsincs, but assume they can be estimated for each frame. Neither do we assume ground-truth object locations, but rely on an off-the-shelf object detector \cite{ren2015faster} to locate the agents in 2D, such as both tennis players.}
% We do not require ground-truth camera intrinsics and extrinsincs, but assume they can be estimated for each frame $\langle$\textbf{6}$\rangle$. Finally, we assume there exists an off-the-shelf object detector \cite{ren2015faster} to locate the agents in 2D, such as both tennis players $\langle$\textbf{6}$\rangle$. 

\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize

\begin{tabular}{lp{0.08\textwidth}p{0.35\textwidth}}
\toprule
\bf  &\bf Name& \bf Description\\
\midrule
$\langle$\textbf{1}$\rangle$ &\textit{Playability} & The user can control generation with discrete actions.\\
$\langle$\textbf{2}$\rangle$ & \textit{Camera control} & The camera pose is explicitly controlled at test time.\\
$\langle$\textbf{3}$\rangle$ & \textit{Multi-object}& Each object is explicitly modeled. \\
$\langle$\textbf{4}$\rangle$& \textit{Deformable objects} & The model handles deformable object such as human body\\
$\langle$\textbf{5}$\rangle$ & \textit{Appearance changes} & The appearance of the objects are not constant is the training set \\
$\langle$\textbf{6}$\rangle$ & \textit{Robustness} & The model is robust to calibration and localization errors.\\

\bottomrule
\end{tabular}
\end{center}
\caption{Characteristics of our Playable Environments. Each row is referred in the text with $\langle \cdot \rangle$ symbols.}

\label{table:requirements}
\end{table}
%\vlad{Move this paragraph before the previous one? Otherwise, we talk about our method, then about existing techniques, then about our method again. }  
%\sergey{Actually this is intentional, I thought to introduce the method broadly, explain what we do. At that point the reader might say that other works do that too, hence this paragraphs shows the differences, then we give slightly more details about our method.}

Playable Environments are closely related to several image or video manipulation problems. %Manipulating videos is  a long-standing problem in computer vision and graphics communities. 
%Multiple works attempt it from different perspectives. 
Novel view synthesis and volumetric rendering methods \eli{missign citations} support re-rendering of static scenes. With rare exceptions [] such methods do not support moving or articulated objects \sout{$\langle$\textbf{3}-\textbf{5}$\rangle$} and do not allow user interaction \sout{$\langle$\textbf{1}$\rangle$}. Video synthesis methods manipulate videos by predicting future frames \cite{lee2018savp,kumar2020videoflow,tulyakov2018moco,tian2021good}, animating~\cite{siarohin2019monkeynet,Siarohin2019firstorder,siarohin2021motion} or playing videos \cite{menapace2021pvg} but do not meet several other characteristic of Playable Environments, such as camera control, multi-object support \sout{$\langle$\textbf{2},\textbf{3}$\rangle$} and others. Consequently, these methods limit interactivity as they do not take into account the 3D nature of the environment. 

%\vlad{In the following, NeRF should be introduced with more details by saying smth.~like ``Recently, coordinate-based neural volumentric representations gained attention. They do XXX and enable YYY... This paper adapts/proposes NeRF-based components for ZZZ.'' } 

Our method consists of two components. The first one is the synthesis module. It extracts the state of the environment---location, style and non-rigid pose of each object---and renders the state back to the image space. Recently introduced Neural Radiance Fields (NeRFs)~\cite{mildenhall2020nerf} represent an attractive vehicle for their ability to render novel views. They employ a coordinate-based neural volumentric representation that enables novel view synthesis with an unprecedented quality. In this work, we introduce style-based modulations of NeRF to support objects of different appearances. 
% Instead of rendering radiance directly and similarly to[], we compose image features decoded by a CNN. 
Furthermore, we introduce a compositional non-rigid volumetric rendering approach handling the rigid field and non-rigid objects. 
The second component---the action module---enables playability. It takes two consecutive states of the environment and predicts an action with respect to the camera orientation. We train our framework using reconstruction losses in image space and the state space. Finally, to improve temporal dynamics, we introduce a temporal discriminator that operates on sequences of environment states. 
% 
%To evaluate playability, Menapace et al.~\cite{menapace2021pvg} use a 2D dataset of tennis matches. Since our playable environments are 3D, we introduce 2 newly collected datasets with camera movements. A large scale tennis dataset consisting of 43 tennis matches and the Minecraft Camera dataset. Furthermore, our method unlocks creative applications, such as real-video re-rendering, re-playing, object appearance manipulation and predicting future frames---all in a playable fashion. %The code, data and pre-trained models will be released to the community.
% 
In summary, the primary contributions of this work are as follows: 
\begin{itemize}\itemsep0em  
    \item A new framework for interactive video generation from a single image featuring the six characteristics that define {Playable Environements} (see Tab.~\ref{table:requirements}). 
    \item A new compositional NeRF that handles deformable objects with different visual style and a new training strategy that shows higher video quality and improved  playability. 
    \item Two new large-scale datasets \willi{Can we define the Minecraft dataset large-scale?} that allow training of {Playable  Environments}. 
\end{itemize} 

Experimentally, we perform quantitative and qualitative comparison with several baselines to support objects of different appearances derived from existing NeRF and video generation methods\sergey{$\longleftarrow$ I do not understand}. These experiments show that our methods is able to generate high quality videos and outperforms all baselines in terms of video quality, camera control and playability.

%\vlad{Also currently missing: a short summary of the experimental results. Mention that our method enables functionality which none of the existing techniques can demonstrate. Mention briefly how we compare our method against existing methods, e.g., our method convinces in a user study, etc.} 

%\vlad{Any promise to release the source code and the new dataset?} 

% Can such reasoning be performed by a model trained on a set of diverse videos? In this paper we present a method to do this. At inference time given an image or a video it builds a playable environment that features aforementioned capabilities. Fig X shows an environment constructed by our method. In it, with the help of a set of actions the user a set of actions to move tennis players, use arrows to move the camera to change a view point and change the style of the player and the field. 




% Capabilities to change, manipulate, re-render and stylize recorded footage  extensive usage in movie and game industry. They require understanding of 

% Contrasting:
% - from volumetric rendering and novel view synthesis
% - from animation
% - from PVG

% From idea to tools, or from existing works by contrast?

% We present a framework 

% Key points:
% - Novel view sytnethsis with dynamic objects
% - Ability to play and control objects
% - Ability to change the style
% - "Do as I say"?

% How about this?

% There should a be good intro paragraph
% Videos represent verbatim recollection of events. They show environments in which they are recorded, with their geometry and style. They include objects that freely move and perform actions. 

% Videos represent events as they happened. It's not about videos, it's about enviroment

% Consider a tennis match. Broadcast involve sophisticated computer graphics to change the camera view, replay key events to create a more dramatic experience. A further interesting this is what could have been happened.



==> resources/ablation_reconstruction_minecraft_qualitatives.tex <==


\begin{figure}
     \centering

     \includegraphics[width=1.0\linewidth]{resources/qualitatives_ablation_reconstruction_minecraft.pdf}
     \caption{Synthesis module reconstruction results on the \emph{Minecraft} dataset. The first image is cropped for better visualization. \emph{Multi}: use of multi-object modeling, $\pi$: use of deformation, $w$: use of style modulation layers or of direct style encoding ($\sim$), $F$: use of the feature renderer or of the simplified renderer ($\sim$).}

    \label{fig:qualitatives_reconstruction_minecraft}
\end{figure}



==> resources/ablation_reconstruction_tennis_qualitatives.tex <==


\begin{figure}
     \centering

     \includegraphics[width=1.0\linewidth]{resources/qualitatives_ablation_reconstruction_tennis.pdf}
     \caption{Synthesis module reconstruction results on the \emph{Tennis} dataset. The image is cropped for better visualization. \emph{Multi}: use of multi-object modeling, $\pi$: use of deformation, $w$: use of style modulation layers or of direct style encoding ($\sim$), $F$: use of the feature renderer or of the simplified renderer ($\sim$).}

    \label{fig:qualitatives_reconstruction_tennis}
\end{figure}

\begin{comment}
\begin{table}
    \centering
    \def\arraystretch{0.0}
    %\resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.0}
    \hspace{-5mm}
    %\resizebox{0.607\linewidth}{!}{
    \begin{tabular}{l@{\hskip 1mm}c@{\hskip 1mm}c@{\hskip 1mm}c@{\hskip 1mm}c@{\hskip 1mm}ccc}
    
         Var. & \emph{Comp.} & $\pi$ & $w$ & $F$ &  &  &   \\
         \midrule
         (a) &&&&&
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_1/150_9.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_1/29_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_1/378_0.png} \\
         \hline
         
        (b) &\checkmark&&&&
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_2/150_9.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_2/29_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_2/378_0.png} \\
         \hline
         
         (c) &\checkmark&\checkmark&&&
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_3/150_9.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_3/29_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_3/378_0.png} \\
         \hline
         
         (d) &\checkmark&\checkmark&\checkmark&&
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_4/150_9.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_4/29_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_4/378_0.png} \\
         \hline
         
         (e) &\checkmark&\checkmark&\checkmark&$\sim$&
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_6/150_9.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_6/29_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ablation_6/378_0.png} \\
         \hline
         
         (Full) &\checkmark&\checkmark&\checkmark&\checkmark&
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ours/150_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ours/29_0.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/dataset_reconstructions/tennis/ours/378_0.png} \\
         \hline

    \end{tabular}
    %}
    %}
    \captionof{figure}{.}
    \label{fig:qualitative_bair_tennis_reconstruction}
\end{table}
\end{comment}

==> resources/architecture_details.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/architecture_details_p.pdf}
    \caption{Architecture of the models employed by our method on the \emph{Tennis} dataset. The number in each block indicates the number of output features or the upsampling factor in the case of upsampling operations. Merging of arrows indicates concatenation. The architecture for the encoder $E$ refers to the encoder for the static object models. We adopt a smaller encoder for the players. \emph{G.S.} indicates Gumbel Softmax \cite{jang2017gumbel}; \emph{Pos. Enc.} indicates positional encoding.}
    \label{fig:architecture_details}
\end{figure*}

==> resources/qualitatives_actions.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_actions_p.pdf}
    \caption{Visualization of the learned action space on the \emph{Minecraft} and \emph{Tennis} datasets for our method and the baselines. Each plot shows $\Delta$ movements of the playable objects measured on the ground plane between a pair of successive frames. Colors indicate the different action label that is associated to each movement. `Inferred' movements are measured on the test sequences, thus the plots shows the actions inferred by the action network as a function of the input states. `Generated' movements are measured on the generated sequences, thus the plots show the movement generated by the dynamics network as a response to the current action input. It can be observed that our method produces sharper decision boundaries between the actions associated to movement. In addition, the distribution of `Generated' movements produced as a response to each action input matches the distribution of the `Inferred' movements associated to the same action. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}.}
    \label{fig:qualitatives_actions}
\end{figure*}

==> resources/qualitatives_camera_manipulation_minecraft.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_camera_manipulation_minecraft_p.pdf}
    \caption{Camera manipulation results on the \textit{Minecraft Camera} dataset. Ground truth shows the reference frame, upper rows show camera manipulation results. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}.}
    \label{fig:qualitatives_camera_manipulation_minecraft}
\end{figure*}

==> resources/qualitatives_camera_manipulation_tennis.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_camera_manipulation_tennis_p.pdf}
    \caption{Camera manipulation results on the \textit{Tennis} dataset. Ground truth shows the reference frame, upper rows show camera manipulation results. To highlight camera manipulation errors, we overlay each generated image with the position where the field lines should be synthesized under the manipulated camera pose. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}.}
    \vspace{1cm}
    \label{fig:qualitatives_camera_manipulation_tennis}
\end{figure*}

==> resources/qualitatives_playability_ablation_minecraft.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_playability_ablation_minecraft_p.pdf}
    \caption{Reconstruction results on the \textit{Minecraft} dataset. Starting from the first frame, the dynamics network reconstructs the ground truth video using the sequence of discrete actions inferred by the action network on the original sequence. \emph{Rel.} use of camera relative residual $\Delta$ output, $D$ use of the temporal discriminator, $\mathcal{L}_{\Delta}$: use of the loss for $\Delta$-\emph{MSE}.}
    \label{fig:qualitatives_playability_ablation__minecraft}
\end{figure*}

==> resources/qualitatives_playability_reconstruction_minecraft.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_playability_reconstruction_minecraft_p.pdf}
    \caption{Reconstruction results on the \textit{Minecraft} dataset. Starting from the first frame, the dynamics network reconstructs the ground truth video using the sequence of discrete actions inferred by the action network on the original sequence. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}.}
    \label{fig:qualitatives_playability_reconstruction_minecraft}
\end{figure*}

==> resources/qualitatives_playability_reconstruction_tennis.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_playability_reconstruction_tennis_p.pdf}
    \caption{Reconstruction results on the \textit{Tennis} dataset. Starting from the first frame, the dynamics network reconstructs the ground truth video using the sequence of discrete actions inferred by the action network on the original sequence. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}.}
    \vspace{2cm}
    \label{fig:qualitatives_playability_reconstruction_tennis}
\end{figure*}

==> resources/qualitatives_style_minecraft.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_style_minecraft_p.pdf}
    \caption{Style transfer results on the \textit{Minecraft} dataset. The topmost row shows the target style, the leftmost column shows the image in which the style is injected.}
    \label{fig:qualitatives_style_minecraft}
\end{figure*}

==> resources/qualitatives_style_tennis.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{resources/qualitatives_tennis_style.pdf}
    \caption{Style transfer results on the \textit{Tennis} dataset. The topmost row shows the target style, the leftmost column shows the image in which the style is injected.}
    \label{fig:qualitatives_style_tennis}
\end{figure*}

==> supplementary_datasets.tex <==
\section{Datasets}
\label{sec:datasets}
In this section we describe the proposed \emph{Minecraft} and \emph{Tennis} datasets for the training of playable environments in in Sec.~\ref{sec:minecraft_dataset} and in Sec.~\ref{sec:tennis_dataset} respectively. We also present details for the \emph{Minecraft Camera} dataset in Sec.~\ref{sec:minecraft_camera_dataset} and the \emph{Static Tennis} dataset in Sec.~\ref{sec:static_tennis_dataset}.


\subsection{Minecraft dataset}
\label{sec:minecraft_dataset}

We collect videos where two \emph{Minecraft} players perform a sparring session. To acquire the sequences we build a Minecraft 16.4 \cite{minecraft} plugin based on \cite{replaymod} (GNU GPL v3). The plugin records Minecraft playing sessions and provides a GUI to replay the recorded sessions and render them under arbitrary camera trajectories. In addition, it is possible to re-render each sequence using different sets of textures for the environment and the players. Our plugin complements the rendered video with metadata containing camera intrinsic and extrinsic parameters and information about the entities that are present in the scene (eg. players). We release the code for the modified plugin to foster the use of Minecraft as a research tool.

We acquire sequences under varying illumination conditions where the camera slowly circles in a dome around the sparring area. Scenes at both day and night are recorded. The training set is composed of 69,600 frames in 1024x576 resolution at 20fps, divided in sequences of 400 frames. The test set and the validation set are composed each of 2,960 frames in sequences of 16 frames at 5fps. A total of 16 unique player identities are present. Note that the dataset can be automatically re-generated at arbitrary resolution and framerate.

\subsection{Minecraft Camera dataset}
\label{sec:minecraft_camera_dataset}

In order to evaluate the camera manipulation capabilities of our method, we collect additional \emph{Minecraft} sequences. In each sequence, the camera starts from an initial pose and is then moved in the neighborhood of the original position in a circular pattern to synthesize novel views of the scene. To allow a better evaluation of novel view synthesis, the rendered scene remains unchanged in all the frames. We collect 24 sequences, each of length 16 frames for a total of 384 frames. 

\subsection{Tennis dataset}
\label{sec:tennis_dataset}

\input{tables/tennis_dataset_statistics}

We build a dataset of tennis match videos collected from YouTube. We collect a total of 43 tennis matches, featuring 86 different player appearances. The matches come from the following tournaments: 13 Us Open matches played on a concrete field, 7 Australian Open matches played on a concrete field, 8 Wimbledon matches played on grass, 15 Roland Garros matches played on red ground.
In each original video, we extract portions of the match where the game is actively being played, from the moment of the service to the realization of the point, and discard parts where no action is occurring. We then process such raw sequences to extract camera calibration information and player bounding boxes.

To perform camera calibration, we exploit the known geometry of the tennis field, using the field itself as a calibration pattern. To detect landmarks on the tennis field, we follow \cite{farin2003robustcameracalibration} using the implementation provided in \cite{implementationfarin2003robustcameracalibration} (BSD 3-Clause). Note that camera parameters obtained in this way present noise due to imprecision in the estimation of landmarks on the tennis field. We discard sequences with implausible camera poses or where camera calibration is excessively noisy using variance in the estimated camera position on the field as a noise estimator. In some sequences, camera calibration fails due to the inability to correctly detect the landmarks. This often happens in sequences from Roland Garros where the field lines are frequently covered by red ground and causes a high number of sequences from Roland Garros to be discarded. When possible, we provide camera parameters estimations for frames where landmark detection fails by interpolating the camera parameters of neighboring frames.

To perform player detection, we make use of a pretrained FasterRCNN \cite{ren2015faster} model. We employ the camera calibration parameters obtained in the preceding step to discard detections associated with people other than the players, \emph{i.e.} referees, ball catchers and spectators. We notice that detection is sometimes inaccurate or fails due to the wide range of movements performed by the players. This happens more frequently for the player positioned further from the camera. Similarly to camera calibration, we discard sequences where detection of one of the players presents an excessive number of failures. When possible, in case of failed detections in one frame, we interpolate the detections of neighboring frames to produce an estimated detection.

The sequences where both camera calibration and player detection complete successfully are selected to be part of the dataset. Tab.~\ref{table:tennis_dataset_statistics} shows the duration statistics for the raw sequences before camera calibration and player detection and for the sequences that were successfully processed. A total of 12.6 hours of videos at 5 fps and 512x288 resolution are successfully processed and are organized in our dataset as follows: 212464 frames as training set organized in sequences of variable length, 6000 frames as validation set organized in sequences of 16 frames, and 6384 frames for test divided in sequences of 16 frames. Note that the original videos are in 1920x1080 resolution and 25fps, so the dataset can be automatically re-generated up to such resolution and framerate.

\subsection{Static Tennis dataset}
\label{sec:static_tennis_dataset}
We adopt the \emph{Tennis} dataset of \cite{menapace2021pvg} to compare with previous playable video generation methods. The dataset is composed of video sequences from 2 matches recorded in the same arena and features 4 players with similar appearance. A total of 40 minutes of training videos is present. The validation and the test set are composed respectively of 2800 and 3280 frames divided in sequences of 16 frames acquired at 5fps. In order to satisfy the assumptions of previous methods, the dataset features limited camera movement and each video is cropped to depict only a single player in the lower part of the field.

%\vlad{The Datasets description can be significantly compressed.} 
%\noindent\textbf{Datasets.} We evaluate our method on four video datasets:\\
%\noindent \textbullet~\textit{Minecraft} dataset. We collect a synthetic video dataset with duration of 1h where two \emph{Minecraft} players perform a sparring session. The dataset features wide camera movement and diverse players. % to evaluate camera and style modeling capabilities.

%\noindent \textbullet~\textit{Minecraft Camera} dataset. We collect auxiliary \emph{Minecraft} sequences where the camera is moved in the neighborhood of a starting position. We use the frames obtained in this way as a convenient ground truth to evaluate camera manipulation capabilities.

%\noindent \textbullet~\textit{Tennis} dataset. We collect a large scale dataset of 43 tennis matches totalling 11.8h of videos. The dataset features different tennis fields and players to evaluate style modeling capabilities.

%\noindent \textbullet~\textit{Static Tennis} dataset. We adopt the \emph{Tennis} dataset of \cite{menapace2021pvg} to allow comparison with playable video generation methods. Differently from our \emph{Tennis} dataset, to satisfy the assumptions of previous methods, the dataset features limited camera movement and each video is cropped to depict only a single player.

%The dataset are further detailed in the \emph{Supp. Mat.}.

==> supplementary_experiments.tex <==

\section{Experiments}
\label{sec:experiments}

In this section we show additional experimental results. Our experiments are complemented by a website (see \href{\webpage}{\webpagename}) showing additional video qualitative results including video sequences produced interactively by users,  camera and style manipulation results, and samples of dataset sequences. Sec.~\ref{sec:synthesis_module_user_study} shows a user study for the evaluation of video quality, Sec.~\ref{sec:playability_evaluation} shows additional playability evaluation results, Sec.~\ref{sec:playability_user_study} describes the user study for the evaluation of playability, Sec.~\ref{sec:synthesis_ablation_evaluation} shows ablation results for the synthesis module, Sec.~\ref{sec:action_ablation_evaluation} shows ablation results for the action module, Sec.~\ref{sec:camera_manipulation_evaluation} presents additional results for camera manipulation and Sec.~\ref{sec:style_manipulation_evaluation} shows style manipulation results.

\begin{comment}
\subsection{Evaluation Metrics}
\noindent\textbf{Video quality metrics.}
We adopt \textit{LPIPS}~\cite{zhang2018unreasonable}, \textit{FID}~\cite{heusel2017advances} and \textit{FVD}~\cite{unterthiner2018towards} computed between the test sequences and the reconstructed sequences.

\noindent\textbf{Action space metrics.}
We make use of a pretrained FasterRCNN \cite{ren2015faster} model to detect objects in the reconstructed sequences and combine this information with ground truth object detections to derive a set of metrics evaluating the quality of the relationship between the learned action space and the behavior of the objects in the environment. Given a pair of frames and an object, we define $\Delta$ as the difference in position of that object between the two frames and associate to it the corresponding action inferred by the action network for that frame pair. Note that $\Delta$ can be computed in different spaces such as the 2D image plane or the 3D environment and can be derived using the detections. Detections in both test and reconstructed sequences can be used in the computation of $\Delta$. In the former case, the association between $\Delta$ and the corresponding action captures information about the action learning process, in the latter, it captures the capability of the model to condition the video generation process on actions.  Given a set of $\Delta$ and a corresponding set of actions, we define the following metrics.

\noindent \textbullet~\textit{$\Delta$ Mean Squared Error ($\Delta$-MSE)} \cite{menapace2021pvg}: The expected error in terms of MSE in the regression of $\Delta$ from a discrete action. For each action, the average $\Delta$ is measured and used as the optimal estimator. The metric is then normalized by the variance of $\Delta$.

\noindent \textbullet~\textit{$\Delta$-based Action Accuracy ($\Delta$-Acc)} \cite{menapace2021pvg}: The accuracy with which a discrete action can be regressed from the associated $\Delta$.

Two additional metrics capture both the quality of the action space and video quality

\noindent \textbullet~\textit{Average Detection Distance (ADD)} \cite{menapace2021pvg}: The average Euclidean distance between the bounding box centers of corresponding objects in the test and reconstructed frames, measured in pixels.

\noindent \textbullet~\textit{Missing Detection Rate (MDR)} \cite{menapace2021pvg}: The portion of detections that are present in the test sequences but that are not matched by any detection in the reconstructed sequences


\noindent\textbf{Video quality metrics.}
We adopt \textit{LPIPS}~\cite{zhang2018unreasonable}, \textit{FID}~\cite{heusel2017advances} and \textit{FVD}~\cite{unterthiner2018towards} computed between the test sequences and the reconstructed sequences, focused on the evaluation of $\langle$\textbf{2},\textbf{4}-\textbf{6}$\rangle$.

\noindent\textbf{Action space metrics.}
We define $\Delta$ as the difference in position of an object between two given frames.
%$\Delta$ can be computed using positions in different spaces such as the 2D image plane or the 3D environment.
Given a set of $\Delta$ and a corresponding set of inferred actions, we define the following metrics, aimed at evaluating $\langle$\textbf{1},\textbf{3}$\rangle$.

\noindent \textbullet~\textit{$\Delta$ Mean Squared Error ($\Delta$-MSE)} \cite{menapace2021pvg}: The expected error in terms of MSE in the regression of $\Delta$ from a discrete action. For each action, the average $\Delta$ is used as the optimal estimator. The metric is normalized by the variance of $\Delta$.\\
%
\noindent \textbullet~\textit{$\Delta$-based Action Accuracy ($\Delta$-Acc)} \cite{menapace2021pvg}: The accuracy with which a discrete action can be regressed from the associated $\Delta$.

\noindent\textbf{Action space and video quality metrics.}

\noindent \textbullet~\textit{Average Detection Distance (ADD)} \cite{menapace2021pvg}: The average Euclidean distance between the bounding box centers of corresponding objects in the test and reconstructed frames.\\
%
\noindent \textbullet~\textit{Missing Detection Rate (MDR)} \cite{menapace2021pvg}: The portion of detections that are present in the test sequences but that are not matched by any detection in the reconstructed sequences.
\end{comment}

%\subsection{Comparison on Playable Video Generation: additional details}
%Since the original dataset is cropped on the lower part of the field to depict a single player, we train our method on an uncropped version of the dataset to avoid camera distortions due to image stretching. The reconstructed images are then cropped to the same regions of the original dataset, and evaluation is performed following the protocol of \cite{menapace2021pvg} to ensure fairness. \eli{previous sentence into supmat}

\subsection{Synthesis module User Study}
\label{sec:synthesis_module_user_study}

In order to further evaluate video quality improvements with respect to CADDY \cite{menapace2021pvg}, we run a user study on video quality against \cite{menapace2021pvg} on the \emph{Static Tennis} dataset, the original dataset of \cite{menapace2021pvg}. Note that, for fairness of comparison, we make use of the \emph{Static Tennis} dataset which does not feature the several challenges addressed by our method but not by CADDY \cite{menapace2021pvg}, such as wide camera movements, multiple players and changes in appearance.

We create 206 video pairs with the two methods and ask 3 distinct AMT users to express their preference in terms of video quality between the two videos. 618 votes expressed by 18 distinct AMT users are gathered and assign a preference of 81.6\% to our method.

\subsection{Playability evaluation}
\label{sec:playability_evaluation}
\input{tables/playability_minecraft}

In Tab.~\ref{table:playability_minecraft}, we present playability evaluation results on the \emph{Minecraft} dataset. As for the \emph{Tennis} dataset, our method surpasses the baselines both in terms of video and action quality metrics. In particular, the high variation in camera pose in this dataset is not correctly modeled by the baseline methods which produce irrealistic results. Note that (i) and (iv) show a better $\Delta$-\textit{ACC} than our method which is explained by their learned action space which only discovers a reduced number of action categories as confirmed by the high $\Delta$-\textit{MSE} and by Fig.~\ref{fig:qualitatives_actions}.


We show qualitatives results for both the \emph{Minecraft} and \emph{Tennis} datasets in Fig.~\ref{fig:qualitatives_playability_reconstruction_minecraft} and Fig.~\ref{fig:qualitatives_playability_reconstruction_tennis} respectively. The movements of the players reconstructed by our method match the ones in the ground truth sequence, indicating that a good action representation is learned. In addition, our model synthesizes players performing motions that are more realistic than the ones produced by the baselines.

We show a representation of the learned action space on both the \emph{Minecraft} and \emph{Tennis} datasets in Fig.~\ref{fig:qualitatives_actions}.

\subsection{Playability User Study}
\label{sec:playability_user_study}
To further evaluate the quality of the action space we perform a user study (see Tab.~\ref{table:playability_user_study_tennis_reduced}) on the \emph{Tennis} dataset, following the protocol of \emph{Menapace} \etal~\cite{menapace2021pvg}. We sample a set of 26 frames from the test set and for each frame we produce video continuations conditioned on each learned action. Two separate videos are produced for each initial frame and action, the first cropped on the lower tennis field, the second cropped on the upper tennis field to ensure a single tennis player is depicted in each video. For each produces sequence, we ask 3 \emph{Amazon Mechanical Turk} users to choose which is the performed action between a set of options. We then measure agreement between the users using the Fleiss' kappa measure \cite{fleiss1971measuring} and compute diversity in the generated actions using entropy of user-selected actions. We consider only the baselines with the highest video quality and with the best action space metrics. Our model achieves the best agreement and comparable diversity to the baselines indicating that the model generates videos that are consistently conditioned by the action and that no mode collapse of the learned actions is present.

\input{tables/playability_user_study_tennis_reduced}

\subsection{Synthesis module Ablation Study}
\label{sec:synthesis_ablation_evaluation}

We present ablation study results for the synthesis module on the \emph{Tennis} dataset in Tab.~\ref{table:ablation_reconstruction_tennis_reduced} and present qualitative results in Fig.~\ref{fig:qualitatives_reconstruction_minecraft} and Fig.~\ref{fig:qualitatives_reconstruction_tennis} respectively for the \emph{Minecraft} and \emph{Tennis} datasets. The evaluation confirms the importance of the use of style modulation layers to model appearance changes and of the bending network to model deformations. In addition, without our feature renderer $F$, the model produces blurry results and lacks details such as the wrinkles on the clothes. Introducing the feature renderer $F$ allows the model to be trained on complete patches applying the perceptual loss term. This, in conjunction with the ability of ConvNets to model inter-pixel relationships, enables the model to reduce blur and to generate clothing that contains more detailed wrinkles. We also note that, in some sequences, the feature renderer is capable of generating realistic player shadows in portions of the image that lie outside of the bounding volume $\beta$ for the radiance field of the player. We ascribe this to the capacity of the ConvNet $F$ to model the correlation between the presence of the player and of its shadow.

\input{tables/ablation_reconstruction_tennis_reduced}
\input{resources/ablation_reconstruction_minecraft_qualitatives}
\input{resources/ablation_reconstruction_tennis_qualitatives}

%\subsection{Player control evaluation: additional results}
%Since actions and their effects should be independent from camera movements, we compute $\Delta$ based on the position of the objects in the environment rather than the position of their projection on the image plane which is used in \cite{menapace2021pvg}.

\subsection{Action module Ablation Study}
\label{sec:action_ablation_evaluation}

In Fig.~\ref{fig:qualitatives_playability_ablation__minecraft} we show qualitative results for the action module ablation study on the \emph{Minecraft} dataset. We note that, while method variations that do not use the temporal discriminator $D$ produce player movements closer to the ground truth sequence, they tend to produce less realistic motions for the moving players.

\subsection{Camera manipulation evaluation}
\label{sec:camera_manipulation_evaluation}
\input{tables/camera_manipulation_tennis_reduced}

We evaluate camera manipulation capabilities for our method on the \emph{Tennis} dataset. We consider each test sequence and sample two random camera poses by applying noise to the camera pose parameters in the first frame. We then generate a camera trajectory by interpolating between the two poses and render the sequence from the novel camera trajectory. Note that in the \emph{Tennis} dataset the largest portion of the image is occupied by the field plane. Consequently, we can approximately match each image rendered from the novel trajectory to the corresponding original image by applying a homography. We then compute reconstruction losses between the original and the generated sequence warped according to the corresponding homography. While this evaluation does not account for parts of the image that do not lie on the field plane such as the players, it can be used to detect failure cases. We show the results in Tab.~\ref{table:camera_manipulation_tennis_reduced}. LPIPS, ADD and MDR highlight that our method obtains better consistency than the baselines in the generation of novel camera views. In addition, we show qualitatives in Fig.~\ref{fig:qualitatives_camera_manipulation_minecraft} and Fig.~\ref{fig:qualitatives_camera_manipulation_tennis} respectively for the \emph{Minecraft} and \emph{Tennis} dataset.

\subsection{Style manipulation evaluation}
\label{sec:style_manipulation_evaluation}
In Fig.~\ref{fig:qualitatives_style_minecraft} and Fig.~\ref{fig:qualitatives_style_tennis} we show qualitative style manipulation results obtained with our method. We consider a target style image from which we extract the style code $w$ for each object. We then replace the style code in the environment state extracted from a source image with the target style and re-render the image using the synthesis module. Our method can successfully change the appearance of the players and of the static scene elements.

% TODO comment results for the camera manipulation task on Tennis

%We address this issue with an AMT user study where users are asked to express preference between two corresponding sequences generated from the novel trajectory by different methods. Each video is overlaid with the position that the field lines should occupy under the novel camera view and users are specifically asked to pay attention to whether the overlaid lines match the generated ones.

%\willi{Explain in which space the delta is computed for each dataset}
%\willi{Training of the rcnn on minecraft}

\input{resources/qualitatives_actions}
\input{resources/qualitatives_playability_reconstruction_minecraft}
\input{resources/qualitatives_playability_reconstruction_tennis}
\input{resources/qualitatives_camera_manipulation_minecraft}
\input{resources/qualitatives_camera_manipulation_tennis}

\input{resources/qualitatives_style_tennis}
\input{resources/qualitatives_style_minecraft}

\input{resources/qualitatives_playability_ablation_minecraft}


==> supplementary_intro.tex <==
In this Supplementary Material, we discuss additional implementation details (see Sec.~\ref{sec:implementation}), training details (see Sec.~\ref{sec:training}), provide details on the proposed datasets (see Sec.~\ref{sec:datasets}) and show additional experimental results (see Sec.~\ref{sec:experiments}). This Supplementary Material is complemented by a website (see \href{\webpage}{\webpagename}) showing additional video qualitative results such as sequences produced interactively by users, camera manipulation and style manipulation results. We also submit our code for review which will be made publicly available.

==> supplementary_limitations.tex <==
\section{Discussion}
\label{sec:discussion}
The following section discusses the main limitations of the method and social implications.

\noindent\textbf{Limitations.}  Our method performs some assumptions on the structure of the environment. First, while the appearance of the environment can change, the method assumes a constant geometry of the environment, preventing it from operating on datasets with actions performed in environments with different geometries. Second, in order to estimate the pose of dynamic objects, the method assumes that moving objects are located on the $y=0$ plane. Lastly, while on the \emph{Minecraft} dataset our method is learns a full 3D environment, on the \emph{Tennis} dataset the presence of camera rotations but not of camera translations makes the problem of recovering the field geometry ill-posed. We thus impose a ``flat world'' prior in order to regularize the geometry learned on this dataset, which is detailed in Sec.~\ref{sec:object_configurations}. This prior allows wider camera manipulations at inference time, but has the effect of projecting parts of the background on flat surfaces, causing visual artifacts when the position of the camera differs from the one of the original dataset.

We also note that our method exhibits blur artifacts or missing-part artifacts in regions of the scene corresponding to thin and fast-moving objects such as the limbs of players or the rackets. The challenging nature of the \emph{Tennis} dataset with frequent motion blur, object parts as small as a few pixels (eg. limbs) and noise in camera calibration is the main reason behind these artifacts that are partially addressed by our feature renderer.

When learning actions, it is important to consider both ease of manipulation, and the portion of interesting actions that can be captured. Users are typically mainly interested in manipulating the position of objects which is often correlated to the change in poses. Thus, to ease the manipulation, we found an ideal solution in learning actions related to changes in position and letting the  model  synthesize the corresponding change in poses. The main limitation caused by this tradeoff between action space simplicity and action space expressiveness is that it is difficult to control the synthesis of actions featuring changes in pose that are not directly correlated to changes in position, such as the swing of the racket.

Lastly, we remark that at inference time objects in the scene are animated independently from each other. This can generate artifacts such as both tennis players swinging the rackets at the same time and makes it not possible to capture interactions between objects in the scene.


\noindent\textbf{Social Implications.}  Similarly to methods operating on face and human appearances, our method could be used to deceive, and can potentially be used to tamper video sequences for nefarious purposes. However, we note that the constant environment geometry assumed by the method provides some protection against fraudulent uses since the method requires a certain scene to appear in many videos in the training dataset in order to allow its subsequent manipulation. This would make it not straightforward to tamper an isolated video for which the malicious individual does not dispose of a corresponding collection of videos of the same scene to use for training. We believe that the benefits brought in terms of novel creative applications and enhancements to user creativity outweigh the potential risks.

\begin{comment}
\noindent\textbf{Limitations.} 
% 
Our method % is limited by the 
assumes constant geometry of the environment, preventing it from operating on datasets with actions in different environments. In addition, on the \emph{Tennis} dataset the presence of camera rotations but not of camera translations makes the problem of recovering the field geometry ill-posed and a ``flat world'' assumption is necessary for this dataset (see \emph{Supp. Mat.}).
% 
% In addition, our method performs optimally when actions are linked to movement of the playable objects and has reduced performance in the identification of actions related to change in pose. 
Next, the performance drops when identifying actions related to change in pose. 
% 
% We ascribe this behavior to the increased complexity of actions expressed in the space of poses. 
% 

\noindent\textbf{Social Implications.} 
% 
While, similarly to methods operating on face and human appearances, our method could be used to deceive, we believe that the benefits brought in terms of novel creative applications outweigh the potential risks.
%Though not negligible, the impact of potential misuses of our method is low compared to that of methods operating on face and human appearances.
\end{comment}

==> supplementary_method.tex <==
\section{Implementation Details}
\label{sec:implementation}

In this section, we discuss additional implementation details for our method. Sec.~\ref{sec:intro_nerf} introduces NeRF \cite{mildenhall2020nerf}, Sec.~\ref{sec:architecture_details} discusses the architecture of the models adopted in our method, Sec.~\ref{sec:feature_renderer} discusses the implementation details of our feature renderer ConvNet, Sec.~\ref{sec:object_configurations} describes the organization of the objects of which the environment is composed, Sec.~\ref{sec:model_sharing} describes the sharing strategies that are used to model different instances of the same object class and Sec.~\ref{sec:masking} describes details regarding batch normalization and pooling operations in the action module.

\subsection{Introduction to NeRF}
\label{sec:intro_nerf}
NeRF \cite{mildenhall2020nerf} represents scenes as radiance fields: a 5D continuous function that maps a 3D position and a 2D viewing direction to an emitted color $c$ and an opacity $\sigma$. NeRF parametrizes such function as an MLP.

Given a desired camera perspective, the associated image can be rendered exploiting the radiance field representation \cite{mildenhall2020nerf}. A ray $r$ is traced through each pixel and the associated color is obtained by integration:
\begin{equation}
    C(r) = \int_{t_n}^{t_f} T(t)\sigma(r(t))c(r(t)) dt 
\end{equation}
with
\begin{equation}
    T(t) = \mathrm{exp}\left(-\int_{t_n}^{t} \sigma(r(s)) ds\right)
\end{equation}
where $T(t)$ denotes the accumulated transmittance, and $t_n$ and $t_f$ represent the minimum and maximum distance from the camera in which the integration is performed. In practice, the integral can be approximated through quadrature \cite{mildenhall2020nerf}. $N$ positions along each ray $r$ are sampled and the associated color is computed as
\begin{equation}
    \hat{C}(r) = \sum_{i=1}^{N} T_i (1 - e^{-\sigma_i\delta_i}) c_i
\end{equation}
with
\begin{equation}
    T_i = \mathrm{exp}({-\sum_{j=1}^{i-1} \sigma_j\delta_j})
\end{equation}
where $c$ and $\sigma$ are obtained by querying the MLP and $\delta$ denotes the distance between successive samples.

In order to ease the learning of high frequency details, NeRF employs positional encodings of the 3D position and viewing direction as input to the underlying MLP.
In addition, \emph{Mildenhall} \etal \cite{mildenhall2020nerf} propose a stratified sampling approach which exploits a \emph{coarse} neural radiance field to locate portions of the ray corresponding to visible surfaces and allocates additional samples to the neighborhood of such regions. A \emph{fine} neural radiance field is used to compute the final image using both the initial and the additional sampled locations.

The model is trained using L2 distance between the reconstructed and the ground truth color value for each sampled ray.

\input{resources/architecture_details}
\subsection{Architecture details}
\label{sec:architecture_details}
In this section, we discuss the details of the models employed in our framework. Fig.~\ref{fig:architecture_details} shows the models employed on the \emph{Tennis} dataset.

We make use of positional encodings \cite{mildenhall2020nerf} for both $V$ and the bending network $B$. We use 10 and 6 octaves respectively and use the concatenation of the original vector and the encodings as input. Following \cite{park2021nerfies}, we gradually introduce the positional encodings in $B$ during the first 60.000 training iterations. No viewing direction is given as input to $B$ and $V$ to avoid artifacts when the environment is rendered from a camera pose outside of the training distribution. In addition, to reduce memory consumption, we do not make use of the hierarchical sampling scheme (see Sec.~\ref{sec:intro_nerf}).

We model the action network $A$ following \cite{menapace2021pvg} and make use of gumbel softmax sampling \cite{jang2017gumbel} to obtain discrete action representations. In addition, to foster $A$ in predicting actions that are associated to movement, we use only object positions $x_t$ as input rather than the complete environment state $s_t$.

The temporal discriminator $D$ receives as input the object positions $x$ and object poses $\pi$ and is further conditioned on the actions $a$ and action variabilities $v$ inferred on the ground truth sequence.

We modulate the number of residual blocks in $E$ based on the expected size of the input image crop.

\subsection{Feature Renderer Details}
\label{sec:feature_renderer}
We propose to render feature maps at multiple resolutions into the final image using a ConvNet feature renderer $F$. Our ConvNet accepts feature maps $\{f_i\}_{i=1}^{l}$ at $l$ different resolutions, each associated to a downsampling factor $d_i$. We obtain feature map $f_i$ by integration of the features sampled along the rays corresponding to pixel $I_{mn}$ in the original image, such that
\begin{equation}
\begin{gathered}
    m \in \left\{\frac{d_i}{2} + 1 + kd_i\right\}_{k=0}^{\frac{h}{d_i} - 1}, n \in \left\{\frac{d_i}{2} + 1 + kd_i\right\}_{k=0}^{\frac{w}{d_i} - 1}
\end{gathered}
\end{equation}
where $h$ and $w$ are the image height and width and indexes are expressed starting from 1. The process is illustrated in Fig.~\ref{fig:feature_renderer}. Note that each ray is sampled on a grid where the points are at a vertical and horizontal distance of $d_i$ from one another and at distance $d_i / 2$ from the border (see left of Fig.~\ref{fig:feature_renderer} for a visualization of the sampled positions). Note also that the ray is sampled at the pixel location in the original image that corresponds to the center of the associated local patch that will be synthesized by $F$.

In our implementation, we render two separate feature maps at downsampling factors 8x and 4x (see Fig.~\ref{fig:architecture_details}) to capture details at different scales. Note that this approach allows rendering images using 12.8x fewer rays than NeRF approaches that render each pixel with a separate ray, allowing for important reductions in the use of memory and in computational complexity and enables the model to render large image patches at training time. We experiment with greater downsampling factors, but find that further increasing them causes 3D consistency artifacts.

In the presence of calibration and localization noise during training, we observe that NeRF models tend to generate blurry results which are particularly evident on dynamic objects where calibration and localization errors are compounded with errors in the estimation of the object pose. We ascribe this phenomenon to the use of reconstruction losses based on L2 distance which, in the presence of a color mismatch between the ground truth and the reconstructed pixel caused by input noise, favors the prediction of intermediate color values, generating blur. Using a feature renderer provides two advantages over the traditional approach. First, thanks to convolutional filters, the prediction for the feature associated to the current position can take into account the values of neighboring positions, enabling the model to produce a coherent output. Second, the possibility to render large patches makes it possible to adopt losses different from L2 distance, such as the perceptual loss of \emph{Johnson} \etal \cite{johnson2016perceptual} which penalizes more effectively implausible predictions such as the ones containing blur.

\begin{figure}
     \centering

     \includegraphics[width=1.0\linewidth]{resources/feature_renderer.pdf}
     \caption{Representation of the feature rendering process. We sample points on rays arranged in a grid corresponding to feature map locations, then the sampled points are rendered into feature maps using our NeRF pipeline. The process is repeated to produce feature maps at different resolutions. The feature rendered $F$ uses the rendered feature maps to reconstruct the original image.}

    \label{fig:feature_renderer}
\end{figure}

\subsection{Object Configurations}
\label{sec:object_configurations}
On the \emph{Minecraft} dataset, we model the scene using four objects. The first object models the static scene elements close to the players, the second object models the distant objects and the other two objects model the players. For each ray, we sample 16 positions for the first model, 1 position for the second model and 32 positions for each of the players.

On the \emph{Tennis} dataset, we note that camera movement in the input dataset is mostly limited to camera rotations. Recovering depth information for the static objects is thus an ill-posed problem which requires prior knowledge. Note that this problem is not present for the players since their change of position with respect to the camera allows the learning of depth information. We thus adopt the following objects to model the environment: an object to model the tennis field which is bounded by a box $\beta$ that does not rise above ground level, an object to model the backplate of the tennis field, which is bounded by its box $\beta$ to be a planar surface, and two objects for the players. For each ray, we sample 4 positions for the objects modeling the static scene and 32 positions for each player.

\noindent\textbf{Minecraft Background Modeling}
The \emph{Minecraft} dataset features a challenging environment with distant visible objects. NeRF++ \cite{kaizhang2020nerfplusplus} employs an inverted sphere scene background representation for modeling distant objects. While effective, this parametrization requires a large number of samples to model distant objects, which increases memory consumption. To address this issue, we propose to model background objects using a spheric background representation which requires a single sample for each ray. In particular, we model the spheric background with as an MLP $f = V(d, o)$, receiving as input the direction $d$ and the origin $o$ of the ray, and returning as output the associated feature. We consider the opacity $\sigma$ of the associated feature to always be 1. The parametrization on the ray origin allows the model to simulate the effects of depth on the background objects without requiring multiple samples.

\subsection{Model Sharing}
\label{sec:model_sharing}
Instead of using a synthesis and an action module specific to each object, we note that objects corresponding to the same class can, in principle, be represented by the same model. In particular, in the \emph{Minecraft} dataset, the two players have completely symmetric characteristics, so we model both using a single shared model. While the same observation can be made for the case of the players in the \emph{Tennis} dataset, we found that the synthesis module fails if the same model is used for both players. We explain this behavior by observing that on the \emph{Tennis} dataset the player closest to the camera is always observed from the back, while the player further from the camera is always observed from the front. This asymmetry makes it harder for a model to learn a unified player representation, so we model the players with separate models.

\subsection{Masked Batch Normalization and Pooling}
\label{sec:masking}
In a video sequence, detection may fail in some frames. In the action module, the environment state corresponding to frames with missing detections and the successive ones are replaced with placeholder values. As discussed in Sec.~\ref{sec:action_training}, loss masking is used to prevent effects of placeholder values on training. Nevertheless, the presence of placeholder values may still alter the behavior of the action module by affecting the estimation of batch statistics in batch normalization layers and by affecting the behavior of operations such as global average pooling. To prevent potential undesired effects on training, in the action module we adopt masked versions of batch normalization and of pooling operations that operate by computing statistics only on non-placeholder values.
 
\section{Training details}
\label{sec:training}

In this section, we describe training details for the synthesis (see Sec.~\ref{sec:synthesis_training}) and the action modules (see Sec.~\ref{sec:action_training}).

\subsection{Synthesis module Training Details}
\label{sec:synthesis_training}
We optimize the synthesis module parameters using Adam \cite{kingma2014adam} as optimizer and learning rate $5e-4$. The model is trained for 300.000 iterations and the learning rate is exponentially decayed until $5e-5$ at the end of training. We employ a batch size of 8 video sequences, each with 3 or 4 frames for \emph{Minecraft} and \emph{Tennis} respectively. To better disentangle style from pose (see Sec.~3.3 on the main paper) we do not use consecutive frames for each sequence, but skip 4 and 100 frames between each selected frame respectively for \emph{Minecraft} and \emph{Tennis}.
 
In all the experiments, we consider input images of size 512x288 and we render patches of size 192x192 and 256x256 respectively for \emph{Minecraft} and \emph{Tennis} during training. To improve the quality of playable objects, we sample with increased frequency patches that contain the players.

The total loss is the weighted sum of the perceptual and L2 reconstruction losses in pixel space. We assign a weight of 1.0 to the L2 reconstruction loss and a weight of 0.1 to the perceptual loss term.

The synthesis module is trained on 4x Nvidia RTX 8000. We also train models on 1x Nvidia RTX 8000 on the \emph{Tennis} dataset using a reduced rendered patch size of 160x160 pixels with a small reduction in image quality.

\noindent\textbf{Feature Renderer Pretraining. } While it is possible to learn the feature renderer network $F$ from scratch, we find it beneficial to start training from pretrained weights since this guides the composable NeRF model towards learning features encodings whose mapping to the image space is already known. We obtain these weights with a pretraining process. We add a temporary encoder ConvNet to $F$ and train it as an autoencoder, using the same combination of perceptual and L2 losses used for training of the synthesis module. To avoid disruption of the learned features in the early stage of training of the synthesis module, we freeze $F$ during the first training iterations of the full model and unfreeze it once the composable NeRF model features become close to the ones the temporary ConvNet encoder would have produced.

\subsection{Action module Training Details}
\label{sec:action_training}
For the action module, we make use of Adam \cite{kingma2014adam} as optimizer with $\beta_1=0.5$ and $\beta_2=0.999$, and use a learning rate of $5e-4$. We train the model for 300.000 iterations with an exponentially decayed learning rate which reaches the value of $5e-5$ at the end of training. The action module and the discriminator are optimized in alternation. We regularize the discriminator training using spectral normalization \cite{miyato2018spectral}.

We note that at inference time our autoregressive dynamics network receives as input sequences of reconstructed environment states $\hat{s}_t$ rather than environment states $s_t$ produced by $E$ as happens during training. Following \cite{menapace2021pvg}, to avoid performance degradation at inference time due to this mismatch, we propose to train the action module using as input to the dynamics network encoded environment states for the first $t$ steps and reconstructed environment states for the following ones. In all the experiments we use 4 initial encoded environment states.

In addition, we employ a curriculum learning strategy where we linearly increase the length of the reconstructed sequences during training. In particular, at the beginning of training, sequences of 5 environment states are reconstructed, while at the end of the annealing period at step 25.000 the reconstructed sequence length is set to 9. We use a batch size of 64 sequences.

Following \cite{menapace2021pvg}, we set the number of actions $K$ to 7 for all the experiments.

We set $\lambda_\mathrm{rec}=1.0$, $\lambda_\mathrm{act}=0.15$, $\lambda_{\Delta}=0.1$ and $\lambda_{\mathrm{G}}=0.1$ in the computation of the total loss term.

The action module is trained on 1x Nvidia RTX 8000.

\noindent\textbf{Loss masking.}
During training of the action module, some frames may not contain a valid detection for each playable object. This may be due to the absence of the object in the frame or due to missed detections. We address this issue by computing the loss terms $\mathcal{L}_{\textrm{rec}}$, $\mathcal{L}_{\textrm{act}}$ and $\mathcal{L}_{\Delta}$ by taking into account only the prefix of the input sequence where the object has always been detected.



 %\willi{Describe ray patching for dynamic objects}
 %\willi{Experiments with rendering at increased resolution}
 %\willi{No hierarchical sampling for speed, describe nerf basics more in depth, eg approximation of the integral}
 %\willi{We rotate the bounding boxes to match the camera orientation}

==> tables/ablation_playability_minecraft.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lcccccccccccc}
\toprule
Variant & \emph{Rel.} & $D$ & $\mathcal{L}_{\Delta}$ &  LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & R.$\Delta$-\emph{MSE}$\downarrow$ & R.$\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule
(A) &&&& 0.205 & 17.0 & 334 & 0.903 & 33.9 & 0.986 & 38.4 & 18.7 & \textbf{33.0} \\
(B) &\checkmark&&& \underline{0.204} & 17.0 & \underline{329} & 0.290 & 76.0 & 0.366 & 79.8 & 18.6 & \underline{33.5} \\
(C) &\checkmark&&\checkmark& \textbf{0.203} & \underline{16.9} & 340 & \textbf{0.263} & \textbf{80.0} & \textbf{0.308} & \textbf{86.7} & \textbf{15.4} & 34.0 \\
(D) &\checkmark&\checkmark&& \underline{0.204} & 17.0 & \textbf{323} & 0.289 & 77.0 & \underline{0.338} & \underline{83.6} & \underline{17.8} & 34.3 \\

\midrule

Full &\checkmark&\checkmark&\checkmark& \underline{0.204} & \textbf{16.8} & \underline{329} & \underline{0.271} & \underline{77.7} & 0.347 & 82.3 & \underline{17.8} & 33.9 \\

\bottomrule
\end{tabular}
\end{center}
\caption{Action module ablation results on the \textit{Minecraft} dataset. \emph{Rel.} use of camera relative residual $\Delta$ output, $D$ use of the temporal discriminator, $\mathcal{L}_{\Delta}$: use of the loss for $\Delta$-\emph{MSE}. $\Delta$-\emph{MSE}, $\Delta$-\emph{Acc} and MDR in \%, ADD in pixels.}
%\vspace{-1mm}
\label{table:ablation_playability_minecraft}
\end{table}

==> tables/ablation_reconstruction_tennis.tex <==
\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize
\begin{tabular}{lccccccccc}
\midrule
Var. & \emph{Multi}\,$\langle$\textbf{3}$\rangle$ & $\pi$\,$\langle$\textbf{4}$\rangle$ & $w$\,$\langle$\textbf{5}$\rangle$ & $F$\,$\langle$\textbf{6}$\rangle$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$  & ADD$\downarrow$ & MDR$\downarrow$ \\
\midrule
(a) &&&&& 0.505 & 256.1 & 7011 & (87.9, 56.5) & (90.3, 80.8) \\
(b) &\checkmark&&&& 0.619 & 271.4 & 10697 & (7.14, 0.0) & (99.9, 100.0) \\
(c) &\checkmark&\checkmark&&& 0.624 & 253.5 & 7280 & (3.68, \textbf{1.61}) & (17.3, 39.8) \\
(d) &\checkmark&\checkmark&$\sim$&& 0.319 & 96.3 & 3303 & (88.9, 70.7) & (99.0, 71.8)  \\
(e) &\checkmark&\checkmark&\checkmark&& 0.286 & 39.3 & 638 & (2.18, 4.03) & (5.26, 9.41) \\
(f) &\checkmark&\checkmark&\checkmark&$\sim$& 0.272 & 39.2 & 2678 & (80.9, 12.8) & (98.6, 22.4) \\
\midrule


Full &\checkmark&\checkmark&\checkmark&\checkmark& \textbf{0.167} & \textbf{17.1} & \textbf{497} & (\textbf{1.70}, 3.41) & (\textbf{1.61}, \textbf{6.18}) \\
\midrule
\end{tabular}
\end{center}
\caption{Environment representation model ablation results on the \textit{Tennis} dataset. \emph{Multi}: use of multi-object modeling, $\pi$: use of deformation, $w$: use of $\mathrm{Sty}$ layers or of direct style encoding ($\sim$), $F$: use of the feature renderer or of the simplified renderer ($\sim$). ADD in pixels, MDR in \%. Results in parentheses refer respectively to the player closest and farthest from the camera.}

\label{table:ablation_reconstruction_tennis}
\end{table}

==> tables/ablation_reconstruction_tennis_reduced.tex <==
\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize
\begin{tabular}{lccccccccc}
\midrule
Var. & \emph{Multi}\,$\langle$\textbf{3}$\rangle$ & $\pi$\,$\langle$\textbf{4}$\rangle$ & $w$\,$\langle$\textbf{5}$\rangle$ & $F$\,$\langle$\textbf{6}$\rangle$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$  & ADD$\downarrow$ & MDR$\downarrow$ \\
\midrule
(a) &&&&& 0.505 & 256.1 & 7011 & 72.2 & 85.6 \\
(b) &\checkmark&&&& 0.619 & 271.4 & 10697 & 3.57 & 100.0 \\
(c) &\checkmark&\checkmark&&& 0.624 & 253.5 & 7280 & 2.65 & 28.6 \\
(d) &\checkmark&\checkmark&$\sim$&& 0.319 & 96.3 & 3303 & 79.8 & 85.4  \\
(e) &\checkmark&\checkmark&\checkmark&& 0.286 & 39.3 & 638 & 3.11 & 7.34 \\
(f) &\checkmark&\checkmark&\checkmark&$\sim$& 0.272 & 39.2 & 2678 & 46.9 & 60.5 \\
\midrule


Full &\checkmark&\checkmark&\checkmark&\checkmark& \textbf{0.167} & \textbf{17.1} & \textbf{497} & \textbf{2.56} & \textbf{3.90} \\
\midrule
\end{tabular}
\end{center}
\caption{Synthesis module ablation results on the \textit{Tennis} dataset. \emph{Multi}: use of multi-object modeling, $\pi$: use of deformation, $w$: use of style modulation layers or of direct style encoding ($\sim$), $F$: use of the feature renderer or of the simplified renderer ($\sim$). ADD in pixels, MDR in \%.}

\label{table:ablation_reconstruction_tennis_reduced}
\end{table}

==> tables/camera_manipulation_minecraft.tex <==
\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize
\begin{tabular}{lcccccccc}
\midrule
& \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$  & ADD$\downarrow$ & MDR$\downarrow$ \\
\midrule
CADDY \cite{menapace2021pvg} (i) &&&& 0.747 & 306 & 11.7 & 95.8 \\
CADDY \cite{menapace2021pvg} (ii) &\checkmark&&& 0.762 & 324 & 44.7 & 92.2 \\
CADDY \cite{menapace2021pvg} (iii) &\checkmark&\checkmark&& 0.669 & 244 & 29.2 & 82.0 \\
CADDY \cite{menapace2021pvg} (iv) &\checkmark&&\checkmark& 0.699 & 314 & 62.0 & 89.4 \\
CADDY \cite{menapace2021pvg} (v) &\checkmark&\checkmark&\checkmark& 0.679 & 337 & 19.1 & 93.6 \\
\midrule
Ours &&&& \textbf{0.242} & \textbf{29.2} & \textbf{5.69} & \textbf{8.07} \\
\midrule
\end{tabular}
\end{center}
\vspace{-8pt}
\caption{Camera control evaluation results on the \textit{Minecraft Camera} dataset. \emph{Aux.}: use of bounding boxes and camera pose; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. ADD in pixels, MDR in \%.}

\label{table:camera_manipulation_minecraft}
\end{table}

==> tables/camera_manipulation_tennis.tex <==
\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize
\begin{tabular}{lcccccccc}
\midrule
& \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$  & ADD$\downarrow$ & MDR$\downarrow$ \\
\midrule
(i) &&&& 0.659 & 224 & (43.3, 57.4) & (76.2, 87.8) \\
(ii) &\checkmark&&& 0.623 & 170 & (54.7, 54.6) & (31.7, 35.6) \\
(iii) &\checkmark&\checkmark&& 0.425 & 26.1 & (45.4, 30.7) & (9.77, 19.4) \\
(iv) &\checkmark&&\checkmark& 0.634 & 164 & (57.8, 56.9) & (36.4, 46.9) \\
(v) &\checkmark&\checkmark&\checkmark& 0.574 & 216 & (43.8, 26.2) & (43.5, 89.8) \\
\midrule
Ours &&&& \textbf{0.205} & \textbf{20.5} & (\textbf{15.1}, \textbf{12.6})  & (\textbf{2.30}, \textbf{9.22}) \\
\midrule
\end{tabular}
\end{center}
\caption{Camera control evaluation results on the \textit{Tennis} dataset. \emph{Aux.}: use of bounding boxes and camera pose; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. ADD in pixels, MDR in \%. Results in parentheses refer respectively to the player closest and farthest from the camera.}

\label{table:camera_manipulation_tennis}
\end{table}

==> tables/camera_manipulation_tennis_reduced.tex <==
\begin{table}
\begin{center}
\setlength{\tabcolsep}{1.8pt}
\footnotesize
\begin{tabular}{lcccccccc}
\midrule
& \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$  & ADD$\downarrow$ & MDR$\downarrow$ \\
\midrule
(i) &&&& 0.659 & 224 & 50.4 & 82.0 \\
(ii) &\checkmark&&& 0.623 & 170 & 54.7 & 33.7 \\
(iii) &\checkmark&\checkmark&& 0.425 & 26.1 & 38.1 & 29.2 \\
(iv) &\checkmark&&\checkmark& 0.634 & 164 & 57.4 & 41.7 \\
(v) &\checkmark&\checkmark&\checkmark& 0.574 & 216 & 35.0 & 66.7 \\
\midrule
(Ours) &&&& \textbf{0.205} & \textbf{20.5} & \textbf{13.9}  & \textbf{5.76} \\
\midrule
\end{tabular}
\end{center}
\caption{Camera control evaluation results on the \textit{Tennis} dataset. \emph{Aux.}: use of bounding boxes and camera pose; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. ADD in pixels, MDR in \%.}

\label{table:camera_manipulation_tennis_reduced}
\end{table}

==> tables/playability_minecraft.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lccccccccccc}
\toprule
 & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule
(i) &&&& 0.743 & 288 & 3667 & 1.0 & (100) & \textbf{15.1} & 96.8 \\
(ii) &\checkmark&&& 0.773 & 296 & 2906 & 0.999 & 52.8 &  56.3 & 93.2 \\
(iii) &\checkmark&\checkmark&& 0.677 & 211 & 2213 & 0.998 & 53.7 & 42.5 & 82.9 \\
(iv) &\checkmark&&\checkmark& 0.707 & 275 & 2553 & 0.467 & \textbf{83.3}  & 56.2 & 92.2 \\
(v) &\checkmark&\checkmark&\checkmark& 0.691 & 309 & 2187 & 0.439 & 82.6 & 17.4 & 95.1 \\

\midrule

(Ours) &&&& \textbf{0.204} & \textbf{16.8} & \textbf{329} & \textbf{0.271} & 77.7 & 17.8 & \textbf{33.9} \\

\bottomrule
\end{tabular}
\end{center}
\caption{Comparison with baselines on the \textit{Minecraft} dataset. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. $\Delta$-\emph{MSE}, $\Delta$-\emph{Acc} and MDR in \%, ADD in pixels.}
%\vspace{-1mm}
\label{table:playability_minecraft}
\end{table}

==> tables/playability_tennis.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lcccccccccccc}
\toprule
 & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & R.$\Delta$-\emph{MSE}$\downarrow$ & R.$\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule

(i) &&&& 0.313 & 61.0 & 877 & (0.792, 1.01) & (58.9, 26,2) & (0.655, 1.0) & (66.1, 26.4) & (21.0, 49.2) & (7.51, 66.2) \\
(ii) &\checkmark&&& 0.351 & 69.2 & 1109 & (0.483, 0.701) & (62.9, 56.3) & (0.388, 0.800) & (81.2, 61.2) & (20.8, 37.1) & (5.53, 44.0) \\
(iii) &\checkmark&\checkmark&& 0.213 & \textbf{15.4} & 727 & (0.623, 0.763) & (60.9, 54.0) & (0.362, 0.697) & (82.9, 71.1) & (19.7, 17.6) & (5.34, 18.1) \\
(iv) &\checkmark&&\checkmark& 0.445 & 70.3 & 1568 & (0.443, 1.15) & (69.0, 55.7) & (0.538, 0.870) & (74.5, 68.2) & (23.3, 35.8) & (24.3, 41.7) \\
(v) &\checkmark&\checkmark&\checkmark& 0.534 & 191 & 8083 & (0.427, 0.839) & (68.7, 78.3) & (0.637, 1.32) & (68.2, \textbf{78.3}) & (18.5, 21.8) & (32.6, 88.0) \\

\midrule

Ours &&&& \textbf{0.181} & 17.4 & \textbf{485} & (\textbf{0.275}, \textbf{0.310}) & (\textbf{96.0}, \textbf{95.3}) & (\textbf{0.232}, \textbf{0.419}) & (\textbf{89.2}, 77.2) & (\textbf{15.2}, \textbf{12.8}) & (\textbf{1.84}, \textbf{7.84}) \\

\bottomrule
\end{tabular}
\end{center}
\caption{Comparison with baselines on the \textit{Tennis} dataset. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. $\Delta$-\emph{MSE}, $\Delta$-\emph{Acc} and MDR in \%, ADD in pixels. Results in parentheses refer respectively to the player closest and farthest from the camera.}
%\vspace{-1mm}
\label{table:playability_tennis}
\end{table}

==> tables/playability_tennis_minecraft_merged.tex <==
\begin{table*}[ht]
\begin{center}

\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lccc|ccccccc|ccccccc}
\toprule
\multicolumn{4}{c}{} & \multicolumn{7}{c}{\emph{Minecraft}} & \multicolumn{7}{c}{\emph{Tennis}} \\
\midrule
 & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule
(i) &&&& 0.743 & 288 & 3667 & 1.0 & 100.0 & 67.9 & 99.3 & 0.313 & 61.0 & 877 & (0.792, 1.01) & (58.9, 26,2) & (21.0, 49.2) & (7.51, 66.2) \\
(ii) &\checkmark&&& 0.773 & 296 & 2906 & 1.0 & 51.3 & 92.4 & 97.0 & 0.351 & 69.2 & 1109 & (0.483, 0.701) & (62.9, 56.3)  & (20.8, 37.1) & (5.53, 44.0) \\
(iii) &\checkmark&\checkmark&& 0.677 & 211 & 2213 & 0.999 & 54.3 & 82.2 & 96.9 & 0.213 & \textbf{15.4} & 727 & (0.623, 0.763) & (60.9, 54.0)  & (19.7, 17.6) & (5.34, 18.1) \\
(iv) &\checkmark&&\checkmark& 0.707 & 275 & 2553 & 0.599 & 46.2 & 76.3 & 68.9 & 0.445 & 70.3 & 1568 & (0.443, 1.15) & (69.0, 55.7) & (23.3, 35.8) & (24.3, 41.7) \\
(v) &\checkmark&\checkmark&\checkmark& 0.691 & 309 & 2187 & 0.660 & 48.5 & 71.3 & 84.0 & 0.534 & 191 & 8083 & (0.427, 0.839) & (68.7, 78.3)  & (18.5, 21.8) & (32.6, 88.0) \\

\midrule

Ours &&&& \textbf{0.204} & \textbf{16.8} & \textbf{329} & \textbf{0.271} & \textbf{77.7} & \textbf{17.8} & \textbf{33.9} & \textbf{0.181} & 17.4 & \textbf{485} & (\textbf{0.275}, \textbf{0.310}) & (\textbf{96.0}, \textbf{95.3}) & (\textbf{15.2}, \textbf{12.8}) & (\textbf{1.84}, \textbf{7.84}) \\

\bottomrule
\end{tabular}
\end{center}
\caption{Comparison with baselines on the \textit{Minecraft} and \emph{Tennis} datasets. \emph{Aux.}: use of auxiliary bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. $\Delta$-\emph{MSE}, $\Delta$-\emph{Acc} and MDR in \%, ADD in pixels.}
%\vspace{-1mm}
\label{table:playability_minecraft_tennis_merged}
\end{table*}



==> tables/playability_tennis_minecraft_merged_reduced.tex <==
\begin{table*}[ht]
\begin{center}

\setlength{\tabcolsep}{1.0pt}
\footnotesize
\begin{tabular}{lccc|ccccccc|ccccccc}
\toprule
\multicolumn{4}{c}{} & \multicolumn{7}{c}{\emph{Minecraft}} & \multicolumn{7}{c}{\emph{Tennis}} \\
\midrule
 & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
\midrule
CADDY \cite{menapace2021pvg} (i) &&&& 0.743 & 288 & 3667 & 1.0 & (100.0) & 67.9 & 99.3 & 0.313 & 61.0 & 877 & 0.901 & 42.6 & 35.1 & 36.9 \\
CADDY \cite{menapace2021pvg} (ii) &\checkmark&&& 0.773 & 296 & 2906 & 1.0 & 51.3 & 92.4 & 97.0 & 0.351 & 69.2 & 1109 & 0.592 & 59.6  & 29.0 & 24.8 \\
CADDY \cite{menapace2021pvg} (iii) &\checkmark&\checkmark&& 0.677 & 211 & 2213 & 0.999 & 54.3 & 82.2 & 96.9 & 0.213 & \textbf{15.4} & 727 & 0.693 & 57.5  & 18.7 & 11.7 \\
CADDY \cite{menapace2021pvg} (iv) &\checkmark&&\checkmark& 0.707 & 275 & 2553 & 0.599 & 46.2 & 76.3 & 68.9 & 0.445 & 70.3 & 1568 & 0.797 & 62.4 & 29.6 & 33.0 \\
CADDY \cite{menapace2021pvg} (v) &\checkmark&\checkmark&\checkmark& 0.691 & 309 & 2187 & 0.660 & 48.5 & 71.3 & 84.0 & 0.534 & 191 & 8083 & 0.633 & 73.5  & 20.2 & 60.3 \\

\midrule

Ours &&&& \textbf{0.204} & \textbf{16.8} & \textbf{329} & \textbf{0.271} & \textbf{77.7} & \textbf{17.8} & \textbf{33.9} & \textbf{0.181} & 17.4 & \textbf{485} & \textbf{0.293} & \textbf{95.7} & \textbf{14.0} & \textbf{4.84} \\

\bottomrule
\end{tabular}
\end{center}
\vspace{-8pt}
\caption{Comparison with baselines on the \textit{Minecraft} and \emph{Tennis} datasets. \emph{Aux.}: use of bounding boxes and camera pose; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. $\Delta$-\emph{MSE}, $\Delta$-\emph{Acc} and MDR in \%, ADD in pixels.}
%\vspace{-1mm}
\label{table:playability_minecraft_tennis_merged_reduced}
\end{table*}



==> tables/playability_tennis_with_qualitatives.tex <==
\begin{figure*}[t]
  
  \begin{minipage}[b]{0.59\textwidth}
    \centering
    \setlength{\tabcolsep}{1.0pt}
    \footnotesize
    \begin{tabular}[b]{lcccccccccc}
    %\toprule
    %\multicolumn{4}{c}{} & \multicolumn{7}{c}{\emph{Tennis}} \\
    \toprule
     & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ & $\Delta$-\emph{MSE}$\downarrow$ & $\Delta$-\emph{Acc}$\uparrow$ & ADD$\downarrow$ & MDR$\downarrow$\\
    \midrule
    CADDY \cite{menapace2021pvg} (i) &&&& 0.313 & 61.0 & 877 & 0.901 & 42.6 & 35.1 & 36.9 \\
    CADDY \cite{menapace2021pvg} (ii) &\checkmark&&& 0.351 & 69.2 & 1109 & 0.592 & 59.6  & 29.0 & 24.8 \\
    CADDY \cite{menapace2021pvg} (iii) &\checkmark&\checkmark&& 0.213 & \textbf{15.4} & 727 & 0.693 & 57.5  & 18.7 & 11.7 \\
    CADDY \cite{menapace2021pvg} (iv) &\checkmark&&\checkmark& 0.445 & 70.3 & 1568 & 0.797 & 62.4 & 29.6 & 33.0 \\
    CADDY \cite{menapace2021pvg} (v) &\checkmark&\checkmark&\checkmark& 0.534 & 191 & 8083 & 0.633 & 73.5  & 20.2 & 60.3 \\
    
    \midrule
    
    Ours &&&& \textbf{0.181} & 17.4 & \textbf{485} & \textbf{0.293} & \textbf{95.7} & \textbf{14.0} & \textbf{4.84} \\
    
    \bottomrule
    \end{tabular}
    \captionof{table}{Comparison with baselines on the \emph{Tennis} dataset. \emph{Aux.}: use of bounding boxes and camera pose; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. $\Delta$-\emph{MSE}, $\Delta$-\emph{Acc} and MDR in \%, ADD in pixels.}
    \label{table:playability_tennis}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.39\textwidth}
    \centering
    \includegraphics[trim={0 0mm 0 1.5mm},clip,width=69mm]{resources/qualitatives_playability_reconstruction_tennis_main.pdf}
    \captionof{figure}{Qualitative reconstruction results on the \emph{Tennis} dataset.\\}
    \label{fig:playability_tennis}
  \end{minipage}
\end{figure*}


==> tables/playability_user_study_tennis.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{2.0pt}
\footnotesize
\begin{tabular}{lcccccccc}
\toprule
 & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & Agreement & Diversity & \emph{Other} votes\\
\midrule
(iii) &\checkmark&\checkmark&& \textbf{0.432}, 0.274 & 1.80, 1.74 & 1.06, 2.65 \\
(v)  &\checkmark&\checkmark&\checkmark& 0.310, 0.030 & \textbf{1.81}, 1.60 & 5.47, 43.9 \\

\midrule

(Ours) &&&& \textbf{0.432}, \textbf{0.456} & 1.65, \textbf{1.75} & 0.71, 0.88 \\

\bottomrule
\end{tabular}
\end{center}
\caption{User study results on the \textit{Tennis} dataset. \emph{Aux.}: use of bounding box and camera pose information; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. \emph{Other} votes in \%.} 
%\vspace{-3mm}
\label{table:playability_user_study_tennis}
\end{table}

==> tables/playability_user_study_tennis_reduced.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{2.0pt}
\footnotesize
\begin{tabular}{lcccccccc}
\toprule
 & \emph{Aux.} & \emph{H.Res.} & $\mathcal{L}_{\Delta}$ & Agreement$\uparrow$ & Diversity$\uparrow$ & \emph{Other} votes\\
\midrule
CADDY \cite{menapace2021pvg} (iii) &\checkmark&\checkmark&& 0.353 & \textbf{1.77} & 1.86 \\
CADDY \cite{menapace2021pvg} (v)  &\checkmark&\checkmark&\checkmark& 0.170 & 1.71 & 24.7 \\

\midrule

(Ours) &&&& \textbf{0.444} & 1.7 & 0.80 \\

\bottomrule
\end{tabular}
\end{center}
\vspace{-8pt}
\caption{User study results on the \textit{Tennis} dataset. \emph{Aux.}: use of bounding boxes and camera pose; \emph{H.Res.} use of the high resolution model; $\mathcal{L}_{\Delta}$ use of the loss for $\Delta$-\emph{MSE}. \emph{Other} votes in \%.} 
%\vspace{-3mm}
\label{table:playability_user_study_tennis_reduced}
\end{table}

==> tables/tennis_dataset_statistics.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{2.0pt}
\footnotesize
\begin{tabular}{lccc}
\toprule
Tournament & Raw duration & Processed duration & Success \\
\midrule
Us Open & 23.090 & 20.912 & 90.6 \\
Australian Open & 12.267 & 11.778 & 96.0 \\
Wimbledon & 12.014 & 11.574 & 96.3 \\
Roland Garros & 8.448 & 1.205 & 14.3 \\
\midrule
Total & 55.819 & 45.469 & 81.5 \\

\bottomrule
\end{tabular}
\end{center}
\caption{Statistics on the collected \emph{Tennis} dataset indicating the duration of the collected raw sequences before camera calibration and player detection and the duration of the processed sequences for which camera calibration and player detection was performed successful. Success indicates the success rate in camera calibration and player detection. Dirt on the tennis lines causes a low success rate for Roland Garros sequences. Durations in seconds, success rate in \%.} 
%\vspace{-3mm}
\label{table:tennis_dataset_statistics}
\end{table}
